Covertly Controlling a Linear System

Consider the problem of covertly controlling a linear system. In this problem, Alice desires to control (stabilize or change the parameters of) a linear system, while keeping an observer, Willie, unable to decide if the system is indeed being controlled or not. We formally define the problem, under two different models: (i) When Willie can only observe the system's output (ii) When Willie can directly observe the control signal. Focusing on AR(1) systems, we show that when Willie observes the system's output through a clean channel, an inherently unstable linear system can not be covertly stabilized. However, an inherently stable linear system can be covertly controlled, in the sense of covertly changing its parameter. Moreover, we give direct and converse results for two important controllers: a minimal-information controller, where Alice is allowed to used only $1$ bit per sample, and a maximal-information controller, where Alice is allowed to view the real-valued output. Unlike covert communication, where the trade-off is between rate and covertness, the results reveal an interesting \emph{three--fold} trade--off in covert control: the amount of information used by the controller, control performance and covertness. To the best of our knowledge, this is the first study formally defining covert control.

==> old_objectives.tex <==
\subsection{Objectives}
\label{Introduction:Research_objectives}
In covert control the focus is on implementation of ideas from control theory in the realm of information theory, i.e., to control or stabilize a system using an appropriate amount of information about the system state, yet without being detected.
\cref{fig:Covert_Control}, conceptually presents the model we will investigate. It is shows a stochastic system with inherent disturbance (noise), a controller managed by Alice, and an observer Willie.

The questions that arises in this scenario are:
How to model this problem of controlling the system covertly? 
In which circumstances the warden will detect or not, the act of controlling or stabilizing? 
What are the performance of specific controllers?
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{Covert_Control3.pdf}
\caption{A basic Covert Control model. 
Alice observes the system's output, and wishes to control the system, either using a desired reference signal or without it. She can decide how frequently and how accurately to sample the output on the one hand, and how frequent and how strong will be her control signal, on the other. The control signal is an input to the system, but it is also observed by Willie directly (a) or by observing the output of the system (b) (either cleanly or via a noisy channel). Alice's goal is to control the system without being noticed (e.g., stabilize an otherwise unstable system), while Willie's goal is to detect if Alice is indeed controlling the system.}
\label{fig:Covert_Control}
\end{figure}

\subsubsection{Covertly Controlling A Linear System} 
Our investigation concerning a simple linear model, given as follow
\begin{align}\label{eq:simple_linear_model}
\begin{split}
X_{n+1} = a X_{n} + Z_{n} - U_{n},
\end{split}
\end{align}

where $X_{n}$ represents the system state, while $a$ is the system's gain and $Z_{n}$ is the noise (disturbance). 
The obvious questions regarding \cref{eq:simple_linear_model} are: What Willie observes and what are his limitations? What Alice is actually doing in order to control the system and what her goal is? What are the relevant measures?

%Before we move to answer those questions, let us 
Assume for now that $U_{n} = 0$. With bounded noise, if $|a| < 1$ the system is stable.
However, Alice can intervene in the system operation as she desire. If $|a| > 1$ the system is not stable, yet a control signal $U_{n}$ can stabilize it. The game is now as follows: Alice can view $X_{n}$, and produce $U_{n}$ in order to stabilize (or control) the system. Willie, the warden, observes the control signal, $U_{n}$, or the system state signal, $X_{n}$ (or a noisy version of them), and wishes to detect if the system is indeed controlled by such an input signal or not.

Clearly, the model can be extended in numerous directions, yet, as is, it already reveals the tension in covert control: on the one hand, Alice can get a relatively small amount of information on $X_{n}$, and stabilize the system using large corrections. This way, she will prob $X_{n}$ using fewer bits, yet her actions will be easily detected. However, maybe Alice can invest more on probing and computing, and stabilize the system using smaller corrections. In fact, there are several control schemes for such a system. However, when considering covert control, we must focus on manifold of new metrics: the amount of information required by Alice, her ability to perform the control with a low probability of detection, and, possibly, her ability to hide not only the control signal itself, but maybe also its marginal effects on other variables in the system. We can thus put forth the following goal.

\emph{Identify the triangular (information-control-covertness) trade-off between the information required by Alice in order to covertly control \cref{eq:simple_linear_model}. Suggest achievable schemes which allow for a low probability of detection and derive converse results}.


